Semantics for probabilistic programming: higher-order functions, continuous distributions, and soft constraints

We study the semantic foundation of expressive probabilistic programming languages, that support higher-order functions, continuous distributions, and soft constraints (such as Anglican, Church, and Venture). We define a metalanguage (an idealised version of Anglican) for probabilistic computation with the above features, develop both operational and denotational semantics, and prove soundness, adequacy, and termination. They involve measure theory, stochastic labelled transition systems, and functor categories, but admit intuitive computational readings, one of which views sampled random variables as dynamically allocated read-only variables. We apply our semantics to validate nontrivial equations underlying the correctness of certain compiler optimisations and inference algorithms such as sequential Monte Carlo simulation. The language enables defining probability distributions on higher-order functions, and we study their properties.

==> app-examples.tex <==
 % -*- root: lics2016.tex -*-

\todo{More equations here. The goal of this subsection is to show the 
usefulness of our semantics. If this subsection survives, we should try
to make the subsection meet the goal. One way is to have more interesting
examples, such as the first-order equations for SMC and the local posterior
calculation via Conjugate prior. Another is to show something strange, such
as the failure of posterior inference using Hongseok's example.} 

\todo{Argue why it is worth studying higher order functions. Expectation of a nonnegative function wrt. a higher-order distribution.}
\begin{verbatim}
lambda t : T(A) x (A=>R).
case
  norm(let a = force(pi0(t)) in score(pi1(t)(a)))
  of (0,(r,y)) => r
  |  (1,_) => 0.0
  |  (2,_) => 0.0
\end{verbatim}


==> app-proofs.tex <==
% -*- root: lics2016.tex -*-

For the higher-order denotational semantics to be well-defined, we need to interpret the first-order language in a small category of measurable spaces. That is, we need a set, rather than a proper class, of measurable spaces that is closed under countable sums, finite products, the monad $P$, and the density functor, and that contains $\mathbb{R}$. 
\emph{Standard Borel spaces}~\cite{berberian:borel,srivastava:borel} %, which carry the smallest $\sigma$-algebra on the family of open sets of a Polish space, 
almost fit the bill: the only thing we cannot prove is that they allow continuous densities, \ie that they are closed under the density functor~\eqref{eq:dens}. 
%If $X$ is a compact Polish space, then $\Dens(X)$ is again Polish, but not necessarily compact anymore. 
We leave identifying a concrete set of measurable spaces for future investigations, and content ourselves with its existence.

\begin{proposition}
  There is a small full subcategory $\Meas$ of the category of all measurable spaces and measurable functions that contains $\mathbb{R}$, and is closed under countable sums, finite products, the monad $P$, and the functor $\Dens$. 
  % We call its objects \emph{small measurable spaces}.
\end{proposition}
\begin{proof}
  Let $\mathbf{C}_0$ be the set $\{\mathbb{R}\}$.
  For an ordinal number $\alpha$, define
  \begin{align*}
    \mathbf{C}_{\alpha+1} 
    \defeq \mathbf{C}_\alpha 
    & \cup \{ \coprod_{i \in \N} C_i \mid C_i \in \mathbf{C}_\alpha \} \\
    & \cup \{ \prod_{i=1^n} C_i \mid C_i \in \mathbf{C}_\alpha, n \in \N \}\\
    & \cup \{ \Dens(C), P(C) \mid C \in \mathbf{C}_\alpha\},
  \end{align*}
  and for a limit ordinal $\alpha$, define
  \[
    \mathbf{C}_{\alpha} \defeq \bigcup_{\beta < \alpha} \mathbf{C}_\beta.
  \]
  Write $\aleph_1$ for the first cardinal number after $\omega$, the countable cardinal number, and regard $\aleph_1$ as an initial ordinal. 
  We will show that the set $\mathbf{C}_{\aleph_1} = \bigcup_{\alpha < \aleph_1} \mathbf{C}_\alpha = \bigcup_{\alpha \leq \omega} \mathbf{C}_\alpha$ is closed under the desired operations; letting it be the set of objects of $\Meas$ then proves the proposition.
  If $C \in \mathbf{C}_{\aleph_1}$, then $C \in \mathbf{C}_\alpha$ for some countable $\alpha$. Thus $\Dens(C) \in \mathbf{C}_{\alpha+1}$, and since $\alpha+1$ is still countable $\Dens(C) \in \mathbf{C}_{\aleph_1}$. The same goes for $P(C)$. 
  Now let $C_n \in \mathbf{C}_{\aleph_1}$ for all $n \in \mathbb{N}$. Say $C_n \in \mathbf{C}_{\alpha_n}$ for countable ordinals $\alpha_n$. Then $\alpha = \sup_{n \in \mathbb{N}} \alpha_n$ is still countable, and $C_n \in \mathbf{C}_{\alpha}$ for each $n \in \mathbb{N}$. Hence $\prod_{n \in \mathbb{N}} C_n, \coprod_{n \in \mathbb{N}} C_n \in \mathbf{C}_{\alpha+1} \subseteq \mathbf{C}_{\aleph_1}$.
\end{proof}

A similar proof shows that the first-order language of Section~\ref{sec:fo-lang} has at most countably many types. 
Therefore the terms form a set, rather than a proper class, even though every measurable function between measurable types is a constant term. 
Thus the measurable spaces $\ConZ\bA$ of Section~\ref{sec:fo-opsem} are indeed well-defined.


